QUART-Online: Latency-Free Large Multimodal Language Model for Quadruped Robot Learning

This paper addresses the inherent inference latency challenges associated with deploying multimodal large language models (MLLM) in quadruped vision-language-action (QUAR-VLA) tasks. Our investigation reveals that conventional parameter reduction techniques ultimately impair the performance of the language foundation model during the action instruction tuning phase, making them unsuitable for this purpose. We introduce a novel latency-free quadruped MLLM model, dubbed QUART-Online, designed to enhance inference efficiency without degrading the performance of the language foundation model. By incorporating Action Chunk Discretization (ACD), we compress the original action representation space, mapping continuous action values onto a smaller set of discrete representative vectors while preserving critical information. Subsequently, we fine-tune the MLLM to integrate vision, language, and compressed actions into a unified semantic space. Experimental results demonstrate that QUART-Online operates in tandem with the existing MLLM system, achieving real-time inference in sync with the underlying controller frequency, significantly boosting the success rate across various tasks by 65%. Our project page is https://quart-online.github.io.

==> includes/8_app.tex <==
\appendix
\normalsize

\input{includes/apps/prompt_engineering}
\input{includes/apps/method_prompts}

\input{includes/apps/exps_language_vs_code}
\input{includes/apps/exps_human_eval}
\input{includes/apps/exps_robo_code_gen}

\input{includes/apps/exps_reactive_controllers}

\input{includes/apps/vlm}
\input{includes/apps/exps_drawing}
\input{includes/apps/exps_tabletop_real}
\input{includes/apps/exps_mobile_robot}

\input{includes/apps/exps_tabletop_sim}
\input{includes/apps/exps_additional_capabilities}
\input{includes/apps/exps_cross_embodiment}

==> includes/apps/exps_additional_capabilities.tex <==
\subsection{Additional LLM Capabilities} \label{app:additional_capabilities}

Using a large pretrained LLM also means we can leverage its capabilities beyond code-writing.
For example, Code as Policies can parse commands from non-English languages as well as emojis.
See Figure~\ref{fig:additional_capabilities}.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{ims/additional_capabilities.png}
%     \caption{
%     \footnotesize
%     LMPs inherit benefits of LLMs, such as parsing commands from non-English languages and emojis.
%     }
%     \label{fig:additional_capabilities}
% \end{figure}



==> includes/apps/exps_cross_embodiment.tex <==
\subsection{Cross Embodiment Example} \label{app:cross-embod}

CaP exhibit a degree of cross-embodiment support \cite{zakka2022xirl,ganapathi2022implicit} by performing the same task differently depending on the action APIs.
In the example below, we give Hints of the action APIs, and the resultant plan changes depending on the whether or not the robot is omnidirectional or unidirectional.
We note that this ability is brittle with existing LLMs and cannot reliably adapt to APIs that are very different.
More robustness may require larger ones trained on domain-specific code. 

% \lmp{
% \prompt{
% \# omnidirectional robot.\\
% \# available actions: move_up(dist), move_right(dist), move_back(dist).
% }\\
% \query{\# make a U shape 5 meters wide and 10 meters long.}\\
% \resp{\hlcoderesp{robot.move_back(dist=10)}\\
% \hlcoderesp{robot.move_right(dist=5)}\\
% \hlcoderesp{robot.move_up(dist=10)}
% }\\
% \prompt{
% \# unidirectional robot.\\
% \# available actions: turn_left(deg), move_forward(dist).
% }\\
% \query{\# make a U shape 3 meters wide and 8 meters long.}\\
% \resp{\hlcoderesp{robot.move_forward(dist=8)}\\
% \hlcoderesp{robot.turn_left(deg=90)}\\
% \hlcoderesp{robot.move_forward(dist=3)}\\
% \hlcoderesp{robot.turn_left(deg=90)}\\
% \hlcoderesp{robot.move_forward(dist=8)}}
% }

==> includes/apps/exps_drawing.tex <==
% \subsection{Whiteboard Drawing} \label{app:tabletop_shape_drawing}

% In this domain, a UR5e robot is tasked to draw and erase various shapes described by natural language on a whiteboard.
% A dry-erase marker is rigidly attached to the robot end-effector.
% The whiteboard dimensions, location, and the location of the eraser are known.
% Additional objects may be added to the scene for the commands to refer to (\eg draw a circle around the blue block).
% In our demos, we use Google Cloud's speech-to-text and text-to-speech APIs to allow users interact with the system through voice commands and also hear the robot's responses to commands.

% \textbf{Prompts.}
% \begin{raggedright}
% \begin{itemize}
%     \item \code{draw_ui}: the high-level UI for parsing user commands and calling other functions\\
%     \link{https://code-as-policies.github.io/prompts/draw_ui.txt}
%     \item \code{parse_obj_name}: return names of objects from natural language descriptions\\
%     \link{https://code-as-policies.github.io/prompts/parse_obj_name.txt}
%     \item \code{parse_shape_pts}: return sequence of 2D waypoints of shapes from natural language descriptions\\
%     \link{https://code-as-policies.github.io/prompts/parse_shape_pts.txt}
%     \item \code{transform_shape_pts}: performs 2D transforms on a sequence of 2D points from natural language descriptions\\
%     \link{https://code-as-policies.github.io/prompts/transform_shape_pts.txt}
%     \item \code{function_generation}: define functions from comments\\
%     \link{https://code-as-policies.github.io/prompts/fgen_simple.txt}
% \end{itemize}
% \end{raggedright}

% \textbf{APIs.}
% \begin{itemize}
%     \item \code{get_obj_names()} - gets list of available objects in the scene. these are prespecified. 
%     \item \code{get_obj_pos(name)} - get the 2D position of the center of an object by name.
%     \item \code{draw(pts_2d)} - draws a shape by commanding the robot end-effector to follow a squence of points on the whiteboard. The robot first moves to a point above the first point in the trajectory, moves down to until contact with the whiteboard is detected, and proceeds to follow the rest of the trajectory.
%     \item \code{erase(pts_2d)} - erases a shape by commanding the robot end-effector to first establish contact with a eraser (eraser position is hardcoded) before following the the rest of the trajectory.
% \end{itemize}

% \textbf{Instructions.}
% These instructions were given to the robot in series from an initial blank whiteboard.
% See full video and generated code on the website.

% \begin{enumerate}
%     \item draw a 5cm hexagon around the middle
%     \item draw a line that bisects the hexagon
%     \item make them both bigger
%     \item erase the hexagon and the line
%     \item draw the sun as a circle at the top right
%     \item draw the ground as a line at the bottom
%     \item draw a pyramid as a triangle on the ground
%     \item draw a smaller pyramid a little bit to the left
%     \item draw circles around the blocks
%     \item draw a square around the sweeter fruit
% \end{enumerate}



==> includes/apps/exps_human_eval.tex <==
% \subsection{CodeGen HumanEval Additional Results} \label{app:codegen-humaneval-details}

% Here we provide additional results to our HumanEval experiments.
% In total, three variants of the bigger Codex model (code-davinci-002) are tested.
% Our approach is Hier. CodeGen + Hier Prompts, where the prompt encourages the LLM to call yet-to-be-defined functions by including such examples.
% For comparisons, we evaluate against Flat CodeGen + No Prompt, essentially just using the LLM directly, and Flat CodeGen + Flat Prompt, for fair comparison with flat code-generation, since our hierarchical approach has a prompt.
% The prompts only contain only 2 Examples:

% \textbf{Prompt for Flat CodeGen:}
% \lmp{\prompt{
% prompt_f_gen_flat = '''\\
% def get_total(xs: List[float]) -> float:\\
% \atab """Find the sum of a list of numbers called xs.\\
% \atab """\\
% \atab return sum(xs)\\
% \# end of function\\
% \\
% def get_abs_diff_between_means(xs0: List[float], \\
% \atab\atab\atab\atab\atab\atab\atab\atab\atab xs1: List[float]) -> float:\\
% \atab """Get the absolute difference between the means of two\\
% \atab lists of numbers.\\
% \atab m0 = sum(xs0) / len(xs0)\\
% \atab m1 = sum(xs1) / len(xs1)\\
% \atab return abs(m0 - m1)
% \# end of function
% }}

% \textbf{Prompt for Hierarchical CodeGen:}
% \lmp{\prompt{
% def get_total(xs: List[float]) -> float:\\
% \atab """Find the sum of a list of numbers called xs.\\
% \atab """\\
% \atab return sum(xs)\\
% \# end of function\\
% \\
% def get_abs_diff_between_means(xs0: List[float], \\
% \atab\atab\atab\atab\atab\atab\atab\atab\atab xs1: List[float]) -> float:\\
% \atab """Get the absolute difference between the means of two lists of\\
% \atab numbers.\\
% \atab """\\
% \atab m0 = get_mean(xs0)\\
% \atab m1 = get_mean(xs1)\\
% \atab return abs(m0 - m1)\\
% \# end of function
% }}

% Note the only difference in the hierarchical prompt is using a yet-to-be-defined function \code{get_mean} instead of calculating the mean directly.
% This "allows" the LLM to generate code that also call yet-to-be-defined functions.

% We report pass rates for when using the most likely outputs ("greedy", which is done by setting temperature to 0), as well as pass rates for at least one solution from sampling various numbers of solutions (1, 10, and 100) with temperature set to 0.8, similar to those used in prior works~\cite{chen2021evaluating, chowdhery2022palm, xu2022systematic}.

% \begin{table}[ht]
% %   \vspace{0.2em}
%   \setlength\tabcolsep{5.2pt}
%   \centering
%   \caption{
%     \footnotesize
%     Hierarchical code generation also performs better (in \% pass rates) on generic coding problems from the standard HumanEval benchmark~\cite{chen2021evaluating}.
%     For columns, Greedy means decoding LLM with temperature=0, while P@N means evaluating correctness across N samples decoded from LLM with temperature=0.8.
%   }
%     \begin{tabular}{lllll}
%     \toprule
%                                         & Greedy & P@1 & P@10 & P@100 \\
%     \midrule
%     code-davinci-001~\cite{chowdhery2022palm}  & -  & 36.0 & - & 81.7 \\
%     PaLM Coder~\cite{chowdhery2022palm} & -  & 36.0 & - & 88.4 \\
%     \midrule
%     Flat CodeGen + No Prompt            & 45.7    & 34.9 & 75.1  & 90.9   \\
%     Flat CodeGen + Flat Prompts         & 50.6    & 36.6 & 77.6  & 93.3   \\
%     Hier. CodeGen + Hier Prompts & \textbf{53.0}    & \textbf{39.8} & \textbf{80.6}  & \textbf{95.7} \\
%     \bottomrule
%     \end{tabular}
%   \label{table:human_eval_full}
% %   \vspace{-1.2em}
% \end{table}

% See results in Table~\ref{table:human_eval}.
% In all instances hierarchical code generation outperforms flat code generation, and the numbers achieved are higher than those reported in recent works~\cite{chen2021evaluating, chowdhery2022palm, xu2022systematic} 
% Note that we use \texttt{code-davinci-002}, while previous works use \texttt{code-davinci-001}, but the relative improvements with hierarchical are consistent across the board.
% Out of the 164 questions in HumanEval, 6.5\% led to hierarchical code generation, but of which both Flat CodeGen variants got 44\% success, while Hier CodeGen code got 56\%.
% While success rate when sampling 100 responses is above 90\% across the board, we note that sampling multiple solutions is not practical for LMPs, which need to perform tasks in a zero-shot manner without engineering prior unit tests.
% As such, for LMPs we always set temperature to 0 and use the most likely output.

==> includes/apps/exps_language_vs_code.tex <==
\subsection{Reasoning with Code vs. Natural Language} \label{app:code-language-benchmark}

To investigate how robot-relevant reasoning through LLMs can be performed with LMPs rather than with natural language, we created
a benchmark that consists of two sets of tasks: (i) selecting objects in a scene from spatial-geometric descriptions, and (ii) selecting position coordinates from spatial-geometric descriptions.
Object selection has 28 questions with commands such as "find the name of the block closest to the blue bowl," where a list of block and bowl positions are provided as input context in the prompt. 
Position selection has 23 questions with commands such as "interpolate 3 points on a line from the cyan bowl to the blue bowl."
An LLM-generated answer for position selection is considered correct if all coordinates are within 1cm of the ground truth.

We evaluate LMPs against two variants of reasoning with natural language: (i) \textbf{Vanilla}, given a description of the setting (\eg list of object positions) and the question, directly outputs the answer (\eg "Q: What is the top-most block?" $\rightarrow$ "A: red block"), and (ii) \textbf{Chain of Thought (CoT)}~\cite{wei2022chain}, which performs step-by-step reasoning given examples of intermediate steps in the prompt (\eg encouraging the LLM to list out y-coordinates of all blocks in the scene before identifying the top-most block).

\begin{table}[ht]
%   \vspace{-.8em}
  \setlength\tabcolsep{5.2pt}
  \centering
  \caption{
  \footnotesize
  Using code for spatial-geometric reasoning yields higher success rate (mean \%) than using vanilla natural language or chain-of-thought prompting.
  }
  \begin{tabular}{lccc}
  \toprule
                  & \multicolumn{2}{l}{Natural Language} & Code       \\
                    \cmidrule(lr){2-3}\cmidrule(lr){4-4}
    Tasks          & Vanilla             & CoT \cite{wei2022chain}           & LMP (ours) \\
\midrule
Object Selection   & 39                  & 68               & \textbf{96}         \\
Position Selection & 30                  & 48               & \textbf{100}         \\
Total              & 35                  & 58               & \textbf{98}         \\
  \bottomrule
  \end{tabular}
  \label{table:reasoning}
%   \vspace{-.6em}
\end{table}

Results in Table~\ref{table:reasoning} show that LMPs achieve accuracies in the high 90s, outperforming CoT, which outperforms Vanilla. CoT enables LLMs to reason about relations and orders (e.g. which coordinate is to the right of another coordinate), but failures occur for precise and multi-step numerical computations.
By contrast, code from LMPs can use Python to perform such computations, and they often leverage external libraries to perform more complex operations (\eg NumPy for vector addition).
CoT and LMPs are not mutually exclusive -- it is possible to prompt "step-by-step" code-generation to solve more complex tasks via CoT, but this is a direction not explored in this work.

==> includes/apps/exps_mobile_robot.tex <==
% \subsection{Mobile Robot} \label{app:mobile_robot}

% The mobile manipulation experiment is set up with robots from 
% \href{https://everydayrobots.com/}{Everyday Robots} navigating and interacting with objects in a real world office kitchen. The robot has a mobile base and a 7DoF arm. For implementing the perception APIs, we mainly use the RGBD camera sensor on the robot. The robot is shown in Fig.~\ref{fig:edr}.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{ims/edr_robot.pdf}
%     \caption{
%   \footnotesize
%   Experiment Setup for mobile manipulation with a \href{https://everydayrobots.com/}{Everyday Robots} robot.
%     }
%     \label{fig:edr}
% \end{figure}

% \textbf{Prompts.}
% \begin{raggedright}
% \begin{itemize}
%     \item \code{mobile_ui}: the high-level UI for parsing user commands and calling other functions\\
%     \link{https://code-as-policies.github.io/prompts/mobile_ui.txt}
%     \item \code{parse_obj_name}: return names of objects from natural language descriptions\\
%     \link{https://code-as-policies.github.io/prompts/mobile_parse_obj_name.txt}
%     \item \code{parse_position}: return a 2D position from natural language descriptions\\
%     \link{https://code-as-policies.github.io/prompts/mobile_parse_pos.txt}
%     \item \code{transform_traj}: performs 2D transforms on a sequence of 2D points from natural language descriptions \\
%     \link{https://code-as-policies.github.io/prompts/mobile_transform_traj.txt}
%     \item \code{function_generation}: define functions from comments\\
%     \link{https://code-as-policies.github.io/prompts/fgen_simple.txt}
% \end{itemize}
% \end{raggedright}

% \textbf{APIs.}
% \begin{itemize}
%     \item \code{get_obj_names()} - gets list of available objects in the scene. these are prespecified. 
%     \item \code{get_obj_pos(name)} - get the 2D position of the center of an object by name.
%     \item \code{is_obj_visible(name)} - returns whether or not the robot sees an object by name.
%     \item \code{get_visible_obj_names()} - returns a list of currently visible object names.
%     \item \code{get_loc_names()} - returns a list of all predefined location names the robot can navigate to.
%     \item \code{get_obj_pos(name)} - gets the 3D location of an object by name. This object must be currently visible.
%     \item \code{get_loc_pos(name)} - gets the 2D location and 1D angle of a predefined location.
%     \item \code{get_robot_pos_and_angle} - gets the current 3D robot position and 1D angle (heading).
%     \item \code{goto_pos(pos_3d)} - navigates to a 3D position by running the robot's internal motion planner.
%     \item \code{goto_loc(name)} - navigates to a location by name by running the robot's internal motion planner.
%     \item \code{pick_obj(name)} - picks up an object by its name. The object must be currently visible. This is implemented as a scripted picking primitive using ViLD object detections.
%     \item \code{place_at_pos(pos_3d)} - places the currently held object at a position.
%     \item \code{place_at_obj(name)} - places the currently held object on top of another object by name.
%     \item \code{say(message)} - uses the robot's speaker to voice out a message.
% \end{itemize}

% Below we list commands that were performed on the mobile robot platform.
% The first are navgiation-related tasks, while the second are manipulation related.
% For the latter manipulation commands, note the ability of CaP to form "short-term memory" by explicitly record variables (in this case, the robot's past positions) in the Python execution scope and referring back them later.
% See videos and generated code on the website.

% \textbf{Mobile Navigation Instructions.}
% \begin{enumerate}
%     \item Moving in a 3m by 2m rectangle around the office chair
%     \item Do that again but rotated 45 degrees clockwise
%     \item Go in a 1.5m square around the barstool as many times as needed, check each step if there is a banana, only stop moving when you see the banana
%     \item Follow the convex hull containing the chairs
%     \item Move back and forth between the table and the countertop 3 times
% \end{enumerate}

% \textbf{Mobile Manipulation Instructions.}
% \begin{enumerate}
%     \item How many snacks are on the table?
%     \item Take the water bottle from the desk and put it in the middle of the fruits on the table
%     \item This is the compost bin
%     \item This is the recycle bin
%     \item This is the landfill bin
%     \item The coke can and the apple are on the table
%     \item Put way the coke can and the apple on their corresponding bins
% \end{enumerate}

==> includes/apps/exps_reactive_controllers.tex <==
% \subsection{CaP: Reactive Controllers for Toy Tasks} \label{app:reactive-controllers}

% LMPs can express reactive controllers, and we demonstrate this on: (i) OpenAI Gym's CartPole balancing and (ii) end-effector position impedance control. Using the same prompt structure, both controllers can be generated zero-shot, reflecting the knowledge already stored in the language model, which can be invoked when the objective is sufficiently specified in the function signature:

% % \begin{wrapfigure}{r}{0.3\linewidth}
% % %   \vspace{-1.7em}
% %   \begin{center}
% %   \noindent\fbox{\parbox{0.88\linewidth}{
% %     \includegraphics[width=1.03\linewidth]{ims/cartpole.pdf}}
% %   }
% %   \end{center}
% % %   \vspace{-0.7em}
% %   \caption{
% %       \footnotesize
% %       LMPs can balance a cartpole.
% %   }
% %   \label{fig:insertion-sixdof}
% %   % https://docs.google.com/drawings/d/1r4S3DNlJkTEOH2-NYgd3VC5MdTVWyPn9jsaunP3-nlU/edit
% % %   \vspace{-1.0em}
% % \end{wrapfigure}

% \lmp{
% \query{
% \# define function: direction = keep_pole_upright_with_pd_control(x,\\
% x_dot, theta, theta_dot).\\
% \# info: direction is 1 if going right, 0 if going left.
% }\\
% \resp{
% def keep_pole_upright_with_pd_control(x, x_dot, theta, theta_dot):\\
% \atab \# define constants.\\
% \atab kp = 1\\
% \atab kd = 1\\
% \atab \# define direction.\\
% \atab direction = 1\\
% \atab \# define error.\\
% \atab error = theta\\
% \atab \# define error_dot.\\
% \atab error_dot = theta_dot\\
% \atab \# define control.\\
% \atab control = kp * error + kd * error_dot\\
% \atab \# define direction.\\
% \atab if control < 0:\\
% \atab\atab direction = 0\\
% \atab return direction
% }
% }
% \noindent The generated LMP expresses a controller that takes as input the position of the cart, angle of the pole, and their velocities, then it balances the pole by actuating the cart below with discrete left or right actions. This controller is only a simple one that requires initialization to be near upright, but it can stabilize an unstable fixed point.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\linewidth]{ims/cartpole.pdf}
%     \caption{
%   \footnotesize
%   LMPs can balance a cartpole
%     }
%     \label{fig:cartpole}
% \end{figure}

% LMPs can likewise be prompted to express impedance control:
% \lmp{
% \query{
% \# define function: tau = ee_impedance_control(x_curr, x_goal, \\
% \atab\atab\atab\atab\atab\atab\atab\atab x_dot, K_x_mat, D_x_mat, J).
% }\\
% \resp{
% def ee_impedance_control(x_curr, x_goal, x_dot, K_x_mat, \\
% \atab\atab\atab\atab\atab\atab\atab\atab D_x_mat, J):\\
% \atab x_err = x_goal - x_curr\\
% \atab x_dot_err = -x_dot\\
% \atab tau = np.matmul(J.T, \\
% \atab\atab\atab np.matmul(K_x_mat, x_err) + np.matmul(D_x_mat, x_dot_err))\\
% \atab return tau
% }
% }
% \noindent to move a robot arm end-effector towards a goal position with joint torques. 
% The controller is functional in that it can control a UR5e robot in PyBullet, but simplified in that it does not compensate for Coriolis or gravity forces.
% Note the need to include extra information about the expected direction output as well as the hint to use PD control in the function signature.
% Without these hints, the resultant function may still look reasonable (e.g. it may output continuous values for control instead of discrete), but it will not work for this specific environment API.
% For the names of the input gains, \code{_mat} was needed for the LMP to treat them as matrices instead of scalars, and \code{_x} was needed to indicate these gains were for the end-effector, not the joints.
% We demonstrate the use of this controller by commanding the end-effector 3D positions of a UR5e robot in PyBullet.
% The default PD gains of 1 also work in this domain without additional tuning as the CartPole environment is relatively simple.
% More complex continuous control tasks may require actually tuning the gains based on execution feedback, something our method does not support at the moment.

% % For this task, the LMP needs to write a function that moves a robot end-effector from the current position toward a goal position.
% % The input contains current and goal end-effector positions, gains, and a Jacobian matrix.
% % The output is joint torques.
% % This is a simplified impedance controller as it is not instructed to command rotations, and it does not compensate for Coriolis and gravity forces

% Both examples show it is possible to generate simple reactive controllers, but more work is needed to express more complex ones.


==> includes/apps/exps_robo_code_gen.tex <==
\subsection{Robot Code-Generation Benchmark} \label{app:robocodegen-examples}

\subsubsection{Example Questions}
Here are four types of benchmark questions and their examples:
\begin{itemize}[leftmargin=*]
    \item Vector operations with Numpy: \\\code{pts = interpolate_pts_np(start, end, n)}
    \item Simple controls: \\\code{u = pd_control(x_curr, x_goal, x_dot, Kp, Kv)}
    \item Manipulating shapes with shapely: \\\code{circle = make_circle(radius, center)}
    \item Using first-party libraries: \\\code{ret_val = obj_shape_does_not_contain_others(obj_name, other_obj_names)}
\end{itemize}
\noindent For the last type, we provide imports of first-party functions, like ones that get object geometric information by name, as Hints in the prompt.

\subsubsection{Generalization Analysis} \label{app:robocodegen-generalization}

We analyze how well code-generation performs across the fives types of generalizations described in~\cite{hupkes2020compositionality}, where generalization is evaluated by comparing the examples given in the prompt with the new instructions given in the benchmark.
We give a description of the five types of generalization applied to our benchmark.
Specifically, we say that solving a problem in the benchmark demonstrates a particular type of generalization if the problem's instruction or solution satisfy the following conditions:
\begin{itemize}
    \item Systematicity: recompose parts of Examples' instructions or code snippets.
    \item Productivity: have longer code or contains more levels (\eg hierarchical function calls) than Examples.
    \item Substitutivity: use synonyms or replace words of similar categories from Examples.
    \item Localism: reuse seen parts or concepts for different purposes.
    \item Overgeneralization: use new API calls or programming language features not seen in Examples.
\end{itemize}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{ims/generalization_types_flat.png}
%     \includegraphics[width=\linewidth]{ims/generalization_types_hier.png}
%     \includegraphics[width=\linewidth]{ims/generalization_types_improvements.png}
%     \caption{Robot Code-Generation Benchmark Performance across Generalization Types for Flat (top) and Hierarchical (middle) Code-Generation, as well as the performance improvements made by Hierarchical Code-Generation (bottom).}
%     \label{fig:benchmark-generalization}
% \end{figure}
% data: https://docs.google.com/spreadsheets/d/17DNcsPXDhb3hkwWRxj812lUh7cgdxMmE74FsorBPYIg/edit#gid=0
% plots: https://colab.research.google.com/drive/1RXeWbSrmcGXm5op81zxb-5fmKCg7Lf1D?resourcekey=0-EcGD_o2UX3wQCTlXGgaAIA&usp=sharing

In Figure~\ref{fig:benchmark-generalization} we report results across three models.
The top plot shows using flat prompts and flat code generation, while the bottom uses hierarchical prompts and hierarchical code generation.
The relative rankings of the three models are consistent across all generalization types, with code-davinci-002 performing the best.
The smallest model, code-cushman-001, performs especially poorly in Productivity and Localism, but it performs much better on Substitutivity.
Indeed, the high Substitutivity performance across all models may indicate that language models are particularly robust to replacing words that have similar meanings or are from similar categories, while generalization to more complex commands (longer answers via Productivity or maintaining local structures via Localism) are more challenging.
Hierarchical code generation also brings significant performance improvements for both davinci models, especially on Productivity, allowing these models to write longer and more multi-layered functions.
However, these improvements are not apparent for cushman, which actually has lower Substitutivity and Localism success rates, suggesting reaching a certain code-generation capability level is needed before Hierarchical Code-Generation can bring further improvements.


==> includes/apps/exps_tabletop_real.tex <==
% \subsection{Real-World Tabletop Manipulation} \label{app:tabletop_manipultion}

% In this domain, a UR5e robot is tasked to manipulate objects on a tabletop according to natural language instructions.
% The robot is equipped with a suction gripper, and it can only perform pick and place actions parameterized by 2D top-down pick and place positions.
% The robot is also expected to answer questions about the scene (\eg how many blocks are there?) by using the provided perception APIs.
% In our demos, we use Google Cloud's speech-to-text and text-to-speech APIs to allow users interact with the system through voice commands and also hear the robot's responses to commands and questions.
% Currently, the prompt only supports having a set of unique objects.
% This is not a limitation of CaP but rather of the perception system - we do not have a good way of persisting the identity of duplicate objects across VLM detections.
% A more sophisticated system of keeping track of the perceived world state can resolve this issue.

% \textbf{Prompts.}
% \begin{raggedright}
% \begin{itemize}
%     \item \code{tabletop_ui}: the high-level UI for parsing user commands and calling other functions\\
%     \link{https://code-as-policies.github.io/prompts/tabletop_ui.txt}
%     \item \code{parse_obj_name}: return names of objects from natural language descriptions\\
%     \link{https://code-as-policies.github.io/prompts/parse_obj_name.txt}
%     \item \code{parse_position}: return a 2D position from natural language descriptions \\
%     \link{https://code-as-policies.github.io/prompts/parse_position.txt}
%     \item \code{parse_question}: return a response (could be a number, a boolean, or a string) to a natural language question \\
%     \link{https://code-as-policies.github.io/prompts/parse_question.txt}
%     \item \code{function_generation}: define functions from comments\\
%     \link{https://code-as-policies.github.io/prompts/fgen.txt}
% \end{itemize}
% \end{raggedright}

% \textbf{APIs.}
% \begin{itemize}
%     \item \code{get_obj_names()} - gets list of available objects in the scene. these are prespecified. 
%     \item \code{get_obj_pos(name)} - gets the 2D position of the center of an object by name.
%     \item \code{is_obj_visible(name)} - checks if an object is visible by name.
%     \item \code{get_bbox(name)} - gets the 2D axis-aligned bounding box of an object by name. This is in robot base coordinates, not in pixels.
%     \item \code{get_segmask(name)} - gets the segmentation mask of an object detection by name. This is in pixels.
%     \item \code{get_color_rgb(name)} - gets the average RGB color of an object detection crop by name.
%     \item \code{get_corner_name(pos_2d)} - gets the name of the corner (\eg top right corner) closest to the 2d point.
%     \item \code{get_side_name(pos_2d)} - gets the name of the side (\eg left side) closest to the 2d point.
%     \item \code{denormalize_xy(normalized_pos_2d)} - converts a normalized 2D coordinate (each value between 0 and 1) to an actual 2D coordinate in robot frame.
%     \item \code{put_first_on_second(obj_name, target)} - picks the first object by name and places it on top of the target by name. The target could be another object name or a 2D position. Picking and placing are done by moving the suction gripper directly on top of the desired positions, moving down until contact is detected, then either engages or disengages the suction cup.
%     \item \code{say(message)} - uses the robot speaker to voice out a message.
% \end{itemize}

% We demonstrate CaP on three domains in the tabletop manipulation setting.
% Instructions of each domain are listed below and were performed in a sequence.
% See full videos and generated code on the website.

% \textbf{Instructions for 4 blocks domain.}
% \begin{enumerate}
%     \item Put the blocks in a horizontal line near the top
%     \item Move the sky-colored block in between the red block and the second block from the left
%     \item Why did you move the green block?
%     \item Which block did you move?
%     \item Arrange the blocks in a square around the middle
%     \item Make the square bigger
%     \item Undo that
%     \item rotate the square by 45 degrees
%     \item Can you throw blocks?
%     \item Move the red block 5cm to the bottom
%     \item Do the same with the other blocks
%     \item Put the blocks on different corners clockwise starting at the top right corner
% \end{enumerate}

% \textbf{Instructions for 3 blocks and 3 bowls domain.}
% \begin{enumerate}
%     \item Put the red block to the left of the rightmost bowl
%     \item Now move it to the side farthest away from it
%     \item How many bowls are to the left of the red block?
%     \item place the blocks in bowls with non matching colors
%     \item put the blocks in a vertical line 20 cm long and 10 cm below the blue bowl
%     \item imagine that the bowls represent a volcano, a forest, and an ocean
%     \item also imagine that the blocks are parts of a building
%     \item now build a tower in the forest
%     \item show me what happens when a volcano erupts over the ocean
% \end{enumerate}

% \textbf{Instructions for fruits, bottles, and plates domain.}
% \begin{enumerate}
%     \item How many fruits are there?
%     \item Tell me their names
%     \item Are there any fruits on the green plate?
%     \item Move all fruits to the green plate and bottles to the blue plate
%     \item Move the smallest fruit back to the yellow plate
%     \item Wait until you see an egg and put it on the green plate
%     \item Put the darkest object in the plate that has the apple
% \end{enumerate}


==> includes/apps/exps_tabletop_sim.tex <==
\subsection{Simulation Tabletop Manipulation Evaluations} \label{app:sim_full_results}

Similar to the real-world tabletop domain, we construct a simulated tabletop environment, in which a UR5e robot equipped with a Robotiq 2F85 jaw gripper is given natural language instructions to complete rearrangement tasks. The objects include 10 different colored blocks and 10 different colored bowls. The proposed CaP is given APIs for accessing a list of present objects and their locations, via a scripted object detector, as well as a pick-and-place motion primitive that are parameterized by either coordinates or object names.

% \textbf{Prompts.}
% \begin{raggedright}
% \begin{itemize}
%     % \item \code{tabletop_ui}: the high-level UI for parsing user commands and calling other functions\\
%     % \link{https://code-as-policies.github.io/prompts/sim_tabletop_ui.txt}
%     % \item \code{parse_obj_name}: return names of objects from natural language descriptions\\
%     % \link{https://code-as-policies.github.io/prompts/sim_parse_obj_name.txt}
%     % \item \code{parse_position}: return a 2D position from natural language descriptions \\
%     % \link{https://code-as-policies.github.io/prompts/sim_parse_position.txt}
%     % \item \code{function_generation}: define functions from comments\\
%     % \link{https://code-as-policies.github.io/prompts/fgen.txt}
% \end{itemize}
% \end{raggedright}

\textbf{APIs.}
\begin{itemize}
    \item \code{get_obj_names()} - gets list of available objects in the scene. these are prespecified. 
    \item \code{get_obj_pos(name)} - gets the 2D position of the center of an object by name.
    \item \code{denormalize_xy(normalized_pos_2d)} - converts a normalized 2D coordinate (each value between 0 and 1) to an actual 2D coordinate in robot frame.
    \item \code{put_first_on_second(obj_name, target)} - picks the first object by name and places it on top of the target by name. The target could be another object name or a 2D position. Picking and placing are done by moving the suction gripper directly on top of the desired positions, moving down until contact is detected, then either engages or disengages the suction cup.
\end{itemize}

We evaluate CaP and the baselines on the following tasks, where each task refers to a unique instruction template (e.g., ``Pick up the <block> and place it in the corner <distance> to the <bowl>'') that are parameterized by certain attributes (e.g., <block>). We split the tasks into the instructions and the attributes to ``seen'' and ``unseen'' categories, where the ``seen'' instructions or attributes are permitted to appear in the prompt or used for training (in the case of supervised baselines). Full list can be found below. Note that we further group the instructions into ``Long-Horizon'' and ``Spatial-Geometric'' task families. The ``Long-Horizon'' instructions are 1-5 in Seen Instructions and 1-3 in Unseen Instructions. The ``Spatial-Geometric'' instructions are 5-8 in Seen Instructions and 4-6 in Unseen Instructions.

\textbf{Seen Instructions.}
\begin{enumerate}
    \item Pick up the <block1> and place it on the (<block2> or <bowl>)
    \item Stack all the blocks
    \item Put all the blocks on the <corner/side>
    \item Put the blocks in the <bowl>
    \item Put all the blocks in the bowls with matching colors
    \item Pick up the block to the <direction> of the <bowl> and place it on the <corner/side>
    \item Pick up the block <distance> to the <bowl> and place it on the <corner/side>
    \item Pick up the <nth> block from the <direction> and place it on the <corner/side>
\end{enumerate}

\textbf{Unseen Instructions.}
\begin{enumerate}
    \item Put all the blocks in different corners
    \item Put the blocks in the bowls with mismatched colors
    \item Stack all the blocks on the <corner/side>
    \item Pick up the <block1> and place it <magnitude> to the <direction> of the <bowl>
    \item Pick up the <block1> and place it in the corner <distance> to the <bowl>
    \item Put all the blocks in a <line> line
\end{enumerate}

\textbf{Seen Attributes.}
\begin{enumerate}
    \item <block>: blue block, red block, green block, orange block, yellow block
    \item <bowl>: blue bowl, red bowl, green bowl, orange bowl, yellow bowl
    \item <corner/side>: left side, top left corner, top side, top right corner
    \item <direction>: top, left
    \item <distance>: closest
    \item <magnititude>: a little
    \item <nth>: first, second
    \item <line>: horizontal, vertical
\end{enumerate}

\textbf{Unseen Attributes.}
\begin{enumerate}
    \item <block>: pink block, cyan block, brown block, gray block, purple block
    \item <bowl>: pink bowl, cyan bowl, brown bowl, gray bowl, purple bowl
    \item <corner/side>: bottom right corner, bottom side, bottom left corner
    \item <direction>: bottom, right
    \item <distance>: farthest
    \item <magnititude>: a lot
    \item <nth>: third, fourth
    \item <line>: diagonal
\end{enumerate}

In Table~\ref{table:sim_detailed} we provide detailed simulation results that report task success rats for fine-grained task categories.
Attributes refer to \textless{}\textgreater{} fields, the values of which can be seen by the method (\eg training set for CLIPort, prompt for language-based methods).
Instructions refer to the templated instruction type given in each row, which can also be seen or unseen.
A total of 50 trials are performed per task, each with sampled attributes and initial scene configurations (block and bowl types, numbers, and positions).
Note that CLIPort by itself (no oracle) is just a feedback policy and it does not know when to stop --- in this case we run 10 actions from the CLIPort policy and evaluate success at the end.
To improve CLIPort performance, we use a variant that uses oracle information from the simulation to stop the policy when success is detected (oracle termination).

\begin{table*}[t]
\setlength\tabcolsep{5.2pt}
\centering
\caption{
    \footnotesize
    Detailed simulation tabletop manipulation success rate (\%) across different task scenarios.
}
\begin{tabular}{p{0.45\linewidth}cccc}
\toprule
                                                                                                                                                    & \textbf{CLIPort (oracle termination)}& \textbf{CLIPort (no oracle)} & \textbf{NL Planner} & \textbf{CaP (ours)}\\
\midrule
\textbf{Seen Attributes, Seen Instructions}                                                                                                                                      &  & &  &       \\
Pick up the \textless{}object1\textgreater{} and place it on the (\textless{}object2\textgreater{} or \textless{}recepticle-bowl\textgreater{})                                      & 88                     & 44            & 98        & \textbf{100}\\
Stack all the blocks                                                                                                                                                             & \textbf{98}                     & 4             & 94        & 94 \\
Put all the blocks on the \textless{}corner/side\textgreater{}                                                                                                                   & \textbf{96}                     & 8             & 46        & 92 \\
Put the blocks in the \textless{}recepticle-bowl\textgreater{}                                                                                                            & \textbf{100}                    & 22            & 94        & \textbf{100}\\
Put all the blocks in the bowls with matching colors                                                                                                                             & 12                & 14            & \textbf{100}       & \textbf{100}\\
Pick up the block to the \textless{}direction\textgreater{} of the \textless{}recepticle-bowl\textgreater{} and place it on the \textless{}corner/side\textgreater{}                 & \textbf{100}                    & 80            & N/A          & 72 \\
Pick up the block \textless{}distance\textgreater{} to the \textless{}recepticle-bowl\textgreater{} and place it on the \textless{}corner/side\textgreater{}                         & 92                     & 54            & N/A          & \textbf{98} \\
Pick up the \textless{}nth\textgreater{} block from the \textless{}direction\textgreater{} and place it on the \textless{}corner/side\textgreater{}                                  & \textbf{100}                    & 38            & N/A          & 98 \\
Total                                                                                                                                                                            & 85.8                     & 33.0            & 86.4        & \textbf{94.3} \\
Long-Horizon Total                                                                                                                                                               & 78.8                     & 18.4            & 86.4        & \textbf{97.2} \\
Spatial-Geometric Total                                                                                                                                                          & \textbf{97.3}                     & 57.3            & N/A             & 89.3 \\
\midrule
\textbf{Unseen Attributes, Seen Instructions}                                                                                                                                    &  & &  &       \\
Pick up the \textless{}object1\textgreater{} and place it on the (\textless{}object2\textgreater{} or \textless{}recepticle-bowl\textgreater{})                                      & 12                     & 10            & 98        & \textbf{100}\\
Stack all the blocks                                                                                                                                                             & 96                     & 8             & 96        & \textbf{100}\\
Put all the blocks on the \textless{}corner/side\textgreater{}                                                                                                                   & 0                      & 0             & 58        & \textbf{100}\\
Put the blocks in the \textless{}recepticle-bowl\textgreater{}                                                                                                                   & 46                     & 0             & 88        & \textbf{96} \\
Put all the blocks in the bowls with matching colors                                                                                                                             & 30                     & 26            & \textbf{100}       & 92 \\
Pick up the block to the \textless{}direction\textgreater{} of the \textless{}recepticle-bowl\textgreater{} and place it on the \textless{}corner/side\textgreater{}                 & 0                      & 0             & N/A             & \textbf{60} \\
Pick up the block \textless{}distance\textgreater{} to the \textless{}recepticle-bowl\textgreater{} and place it on the \textless{}corner/side\textgreater{}                         & 0                      & 0             & N/A             & \textbf{100}\\
Pick up the \textless{}nth\textgreater{} block from the \textless{}direction\textgreater{} and place it on the \textless{}corner/side\textgreater{}                                  & 0                      & 0             & N/A             & \textbf{60} \\
Total                                                                                                                                                                            & 23.0                     & 5.5             & 88.0        & \textbf{88.5} \\
Long-Horizon Total                                                                                                                                                               & 36.8                     & 8.8             & 88.0        & \textbf{97.6} \\
Spatial-Geometric total                                                                                                                                                          & 0.0                      & 0.0             & N/A             & \textbf{73.3} \\
\midrule
\textbf{Unseen Attributes, Unseen Instructions}                                                                                                                                  &  &  &  &       \\
Put all the blocks in different corners                                                                                                                                          & 0                      & 0             & 60        & \textbf{98} \\
Put the blocks in the bowls with mismatched colors                                                                                                                               & 0                      & 0             & \textbf{92}        & 60 \\
Stack all the blocks on the \textless{}corner/side\textgreater{}                                                                                                                 & 0                      & 0             & 40        & \textbf{82} \\
Pick up the \textless{}object1\textgreater{} and place it \textless{}magnitude\textgreater{} to the \textless{}direction\textgreater{} of the \textless{}recepticle-bowl\textgreater{} & 0                      & 0             & N/A             & \textbf{38} \\
Pick up the \textless{}object1\textgreater{} and place it in the corner \textless{}distance\textgreater{} to the \textless{}recepticle-bowl\textgreater{}                            & 4                      & 0             & N/A             & \textbf{58} \\
Put all the blocks in a \textless{}line\textgreater{}                                                                                                                            & 0                      & 0             & N/A             & \textbf{90} \\
Total                                                                                                                                                                            & 0.7                      & 0.0             & 64.0        & \textbf{71.0} \\
Long-Horizon Total                                                                                                                                                               & 0.0                      & 0.0             & 64.0        & \textbf{80.0} \\
Spatial-Geometric Total                                                                                                                                                          & 1.3                      & 0.0             & N/A             &\textbf{62.0} \\
\bottomrule
\end{tabular}
\label{table:sim_detailed}
\end{table*}
% https://docs.google.com/spreadsheets/d/1UIst_T2b6JeVFI7eNcw6p38H3e5vPvfubk9L4DncF2Q/edit?resourcekey=0-ilQ-IRqY9nZbfG15HrGxYQ#gid=0

==> includes/apps/method_prompts.tex <==
% \subsection{Method Section Prompts} \label{app:method-prompts}

% \subsubsection{Language-based reasoning} \label{prompt:language-reasoning}
% Full prompt:

% \lmp{
% \prompt{
% objs = ['green block', 'green bowl', 'yellow block', 'yellow bowl']\\
% \# the yellow block.\\
% ret_val = 'yellow block'\\
% \# the blocks.\\
% ret_val = ['green block', 'yellow block']
% }}


% \subsubsection{First-party} \label{prompt:first-party}
% Full prompt:

% \lmp{
% \prompt{
% from utils import get_pos, put_first_on_second\\
% objs = ['gray block', 'gray bowl']\\
% \# put the gray block on the gray bowl.\\
% put_first_on_second('gray block', 'gray bowl')\\
% objs = ['purple block', 'purple bowl']\\
% \# move the purple bowl toward the left.\\
% target_pos = get_pos('purple bowl') + [-0.3, 0]\\
% put_first_on_second('purple bowl', target_pos)
% }
% }

% \subsubsection{Combining language reasoning, third-party, and first-party libraries.} \label{prompt:combine-low-level}
% Full prompt:

% \lmp{
% \prompt{
% import numpy as np\\
% from utils import get_pos, put_first_on_second\\
% objs = ['cyan block', 'cyan bowl', 'pink bowl']\\
% \# put the cyan block in cyan bowl.\\
% put_first_on_second('cyan block', 'cyan bowl')\\
% objs = ['gray block', 'silver block', 'gray bowl']\\
% \# place the top most block on the gray bowl.\\
% names = ['gray block', 'silver block']\\
% positions = np.array([get_pos(name) for name in names])\\
% name = names[np.argmax(positions[:,1])]\\
% put_first_on_second(name, 'gray bowl')\\
% objs = ['purple block', 'purple bowl']\\
% \# put the purple bowl to the left of the purple block.\\
% target_pos = get_pos('purple block') + [-0.3, 0]\\
% put_first_on_second('purple bowl', target_pos)
% }\\
% }

% \subsubsection{LMPs can be composed.} \label{prompt:compose-lmp}
% Full prompt:

% \lmp{
% \prompt{
% import numpy as np\\
% from utils import get_pos, put_first_on_second, parse_obj\\
% objs = ['yellow block', 'yellow bowl', 'gray block', 'gray bowl']\\
% \# move the sun colored block toward the left.\\
% block_name = parse_obj('sun colored block')\\
% target_pos = get_pos(block_name) + [-0.3, 0]\\
% put_first_on_second(block_name, target_pos)\\
% objs = ['white block', 'white bowl', 'yellow block', 'yellow bowl']\\
% \# place the block closest to the blue bowl on the other bowl.\\
% block_name = parse_obj('the block closest to the blue bowl')\\
% bowl_name = parse_obj('a bowl other than the blue bowl')\\
% put_first_on_second(block_name, bowl_name)}
% }

% \subsubsection{parse_obj prompt.} \label{prompt:parse-obj}
% Full prompt:

% \lmp{
% \prompt{
% import numpy as np\\
% from utils import get_pos\\
% objs = ['brown bowl', 'green block', 'brown block', 'green bowl']\\
% \# the blocks.\\
% ret_val = ['brown block', 'green block']\\
% \# the sky colored block.\\
% ret_val = 'blue block'\\
% objs = ['orange block', 'cyan block', 'purple bowl', 'gray bowl']\\
% \# the right most block.\\
% block_names = ['orange block', 'cyan block']\\
% block_positions = np.array([\\
% \atab\atab\atab\atab\atab get_pos(block_name) for block_name in block_names])\\
% right_block_name = block_names[np.argmax(block_positions[:, 0])]\\
% ret_val = right_block_name
% }
% }

==> includes/apps/prompt_engineering.tex <==
\subsection{Prompt Engineering} \label{app:prompt-engineering}

Using LMPs to reliably complete tasks via code generation requires careful prompt engineering.
While these prompts do not have to be long, they do need to be relevant and specific.
Here, we discuss a few general guidelines that we followed while developing prompts for this paper.

It is very important for prompts to contain code that \textit{has no bugs}.
Bugs in the prompt lead to unreliable and incorrect responses.
Conversely, if the LMP is writing incorrect code for a given Instruction, the prompt engineer should first verify that the prompt, especially the Examples most closely related to the Instruction, is bug-free.
To reduce bugs related to syntax errors, one simple method is writing prompts in a code editor with syntax highlighting.

There are many cases where the prompt contains variables or functions whose names are ambiguous.
To produce reliable responses under these conditions, Examples in the prompt should treat these ambiguities consistently.
If a variable named \code{point} is treated as an \code{numpy.ndarray} object in one Example and as a \code{shapely.geometry.Point} object in another, the LMP will not be able to ``decide" on which convention to use, resulting in unreliable responses.
Another way to handle ambiguity is by providing informal type hints, such as appending \code{_np} to variable names to indicate its type, or appending it to function names to indicate the type of the returned variable.
In general, more specific variable and function names give more consistent results.

For using third party libraries, including import statements in the prompt may not be necessary, as we found that LMPs can generate code that calls NumPy and SciPy without them.
However, explicit import statements do improve reliability and increase the chance of LMPs using those libraries when the need arises.
For using first party libraries, meaningful function names that follow popular conventions (\eg begin with \code{set_} and \code{get_}) and specify return object formats (\eg \code{get_bbox_xyxy}) induce more accurate usages.
Import statements in the Hints should be formatted as if we were importing functions.
For example, in Python this means using \code{from utils import function_name} instead of \code{import function_name}.
If the latter is used, the LMP may treat the imported name as a package, and the generated code might write \code{function_name.function_name()}.

One type of LMP failures are related to code generation correctness.
For example, minor coding mistakes when calling internal or external APIs, such as missing arguments, can be fixed with an Hint or Example demonstrating the correct usage.
Incorrect assumptions on variable types can also be fixed in similar fashions.
Other coding failures may be addressed by descriptive function names to encourage appropriate library usage (\code{perform_function_with_np()}) or succinct code logic (\code{# implement in one line.})
While it is possible to use LLMs to edit code and fix bugs (\eg by using OpenAI's code edit API), in our experience this yielded inconsistent results (not always able to correct mistakes, and sometimes changed what the function was doing), so we did not employ this method in our experiments.

==> includes/apps/vlm.tex <==
\subsection{Visual Language Models} \label{app:vlm}

For real-world experiments, we use off-the-shelf open-vocabulary object detection models, ViLD~\cite{gu2021open} and MDETR~\cite{kamath2021mdetr} to perform object detection, localization, and segmentation.
These are called visual language models because they take as input a natural language description (caption) of the image and try to find objects in that description.
ViLD is used for the mobile robot domain, while MDETR is used for the tabletop manipulation and whiteboard drawing domains.
Both models give an axis-aligned bounding box in the image along with per-pixel segmentation masks of the detected objects.
To convert these detections to 3D coordinates for both perception and action (\eg scripted picking primitives), we deproject the corresponding pixels from a depth camera, whose transform to the robot frame is registered a priori.
The robustness of today's vision language models could still be improved, and many real-world failures could be attributed to inaccurate detections.
In addition, a degree of prompt engineering is also required for VLMs.
For example, MDETR detects blocks more reliably with the word ``square" than "block," and applying our approach to a new domain will require some prompt engineering for the vision language model.

